VF-Plan: Bridging the Art Gallery Problem and Static LiDAR Scanning with Visibility Field Optimization

Viewpoint planning is critical for efficient 3D data acquisition in applications such as 3D reconstruction, building life-cycle management, navigation, and interior decoration. However, existing methods often neglect key optimization objectives specific to static LiDAR systems, resulting in redundant or disconnected viewpoint networks. The viewpoint planning problem (VPP) extends the classical Art Gallery Problem (AGP) by requiring full coverage, strong registrability, and coherent network connectivity under constrained sensor capabilities. To address these challenges, we introduce a novel Visibility Field (VF) that accurately captures the directional and range-dependent visibility properties of static LiDAR scanners. We further observe that visibility information naturally converges onto a 1D skeleton embedded in the 2D space, enabling significant searching space reduction. Leveraging these insights, we develop a greedy optimization algorithm tailored to the VPP, which constructs a minimal yet fully connected Viewpoint Network (VPN) with low redundancy. Experimental evaluations across diverse indoor and outdoor scenarios confirm the scalability and robustness of our method. Compared to expert-designed VPNs and existing state-of-the-art approaches, our algorithm achieves comparable or fewer viewpoints while significantly enhancing connectivity. In particular, it reduces the weighted average path length by approximately 95%, demonstrating substantial improvements in compactness and structural efficiency. Code is available at https://github.com/xiongbiaostar/VFPlan.

==> 6_acknowledg.tex <==
\section{Acknowledgements}

This work was supported by the National Nature Science Foundation of China (NSFC xxxxxx, NSFC xxxxxx).


==> 7_proof.tex <==
\section{Theoretical Foundations and Global Optimality}\label{sec:theory}

This section formulates the Viewpoint Planning Problem (VPP) for static LiDAR scanning in a 2D polygonal environment and establishes the theoretical basis for restricting candidate viewpoints to the \emph{medial axis} (MA). We first present the problem definition, including coverage and connectivity requirements, and then show that any line segment visible from an interior point is also visible from a corresponding set of MA points. This demonstrates that restricting the viewpoint search space to the MA incurs no loss of coverage capability. Finally, we prove that a minimal solution is \emph{globally optimal} under our MA assumption.

\subsection{Problem Definition}\label{sec:problem_definition}

Let $P$ be a 2D polygonal region (such as a floor plan) with possible obstacles or holes, while remaining topologically connected. The polygon’s boundary (including internal obstacles) is discretized into $n$ small line segments:
\[
L=\{\,l_1,\;l_2,\;\dots,\;l_n\},
\]
which represent the target structures (e.g., walls or windows) to be covered by static LiDAR scanners (hereafter referred to as \emph{viewpoints}).

\paragraph{Candidate Viewpoints}
We aim to position a set of viewpoints such that all segments in $L$ are fully visible, while the chosen viewpoints remain connected under an overlap criterion. Let $V=\{\,v_1,\;v_2,\;\dots,\;v_m\}$ be the set of candidate viewpoint locations. We will later establish that it is sufficient to confine $V$ to the \emph{medial axis} of $P$, reducing a 2D search to a simpler 1D structure.

\paragraph{Visibility} we define a \emph{Completeness Table} $C$, where $C_{ij}$ indicates whether viewpoint $V_i$ observes line segment $L_j$
\begin{equation}\label{eq:completeness}
    C_{ij} = \begin{cases} 
    1 & \text{if } v_i \text{ has an unobstructed view of } l_j \\ 
    0 & \text{otherwise} 
    \end{cases}
\end{equation}

\paragraph{Connectivity via Overlap}
Consider any pair of viewpoints $(v_i, v_k)$. Let $O_{ik}$ be their \emph{overlap ratio}, i.e., the fraction of segments in $L$ that both $v_i$ and $v_k$ can simultaneously observe. For a threshold $\tau$, an edge $(v_i,v_k)$ exists in an \emph{overlap graph} $G=(V,E)$ if $O_{ik}\ge\tau$. A chosen subset $S \subseteq V$ must then form a connected subgraph under this threshold.

\paragraph{Mathematical Formulation}
We seek a minimal subset $S\subseteq V$ of viewpoints such that:
\begin{enumerate}[label=(\alph*)]
    \item \emph{Coverage}: Each segment $l_j\in L$ is observed by at least one viewpoint in $S$, i.e.,
    \begin{equation}\label{eq:coverage}
    \forall\,l_j \in L,\;\exists\,v_i \in S:\;C_{ij}=1.
    \end{equation}
    \item \emph{Connectivity}: The induced subgraph $(S,E_S)$ is connected under the overlap threshold $\tau$, where
    \begin{equation}\label{eq:connectivity}
    E_S \;=\;\bigl\{(v_i,v_k)\in E \;\big\vert\; v_i,v_k\in S,\;O_{ik}\ge\tau\bigl\}.
    \end{equation}
\end{enumerate}

The optimization problem becomes:
\begin{equation}\label{eq:problem_formulation}
\begin{aligned}
\min_{S \subseteq V}\; |S|\quad \text{subject to}\quad 
~\eqref{eq:coverage}\;\text{and}\;~\eqref{eq:connectivity}.
\end{aligned}
\end{equation}

Since problem~\eqref{eq:problem_formulation} generalizes the set cover problem (with additional connectivity constraints), it remains NP-hard. Nonetheless, by restricting $V$ to the medial axis (MA), we retain optimality while reducing the search complexity considerably.

\subsection{Skeleton Completeness and Visibility Propagation}\label{sec:skeleton}

\paragraph{Medial Axis (\emph{MA})}
The MA of $P$ is the set of points inside $P$ that are equidistant to at least two boundary edges. In Blum’s \emph{grassfire transform}~\cite{blum1967}, if the boundary of $P$ is ignited simultaneously, the inward-propagating flames collide and form the locus of the MA.

\begin{theorem}[Skeleton Completeness]\label{thm:extended_skeleton}
Suppose an interior point $p\in P$ sees a set of boundary segments $L_p\subseteq L$. Then there exists a set of points $\{q_l\}\subseteq \mathrm{MA}(P)$ such that
\[
L_p \;\;\subseteq\;\;\bigcup_{l\in L_p}\mathrm{Vis}(q_l).
\]
Hence, for any interior coverage provided by $p$, there exists an MA-based set of points whose collective coverage reproduces that of $p$.
\end{theorem}

\noindent
\textbf{Sketch of Proof.} 
Using Blum’s “fire transformation,” the visibility from every segment propagates inward until it intersects the medial axis $\mathrm{MA}(P)$. Each line segment $l_j\in L_p$ must intersect $\mathrm{MA}(P)$ at some point $q_j$ visible to $l_j$. Thus,
\[
\mathrm{Vis}(p) \;\;\subseteq\;\;\bigcup_{l_j\in \mathrm{Vis}(p)}\,\mathrm{Vis}(q_j).
\]
Consequently, although a single point on the MA may not match $p$’s entire coverage, a suitable collection of MA points can, illustrated in \ref{fig:proof_skeleton}. Restricting $V$ to $\mathrm{MA}(P)$ therefore does not diminish the achievable coverage.

\begin{figure}[!htbp]
    \centering
    \includegraphics[width=\linewidth]{Fig_14_Proof.pdf}
    \caption{%
    Illustration of skeleton completeness. (a) A simple polygon (black boundary) with its medial axis (gray arcs). (b) Coverage by an interior viewpoint \(p\) can be replicated by a single skeletal viewpoint \(q\) lying on the medial axis (MA). (c) In the general case, coverage from an interior viewpoint \(p\) may require multiple skeletal viewpoints (here, \(m\) and \(n\)) to fully reproduce \(p\)'s visibility. Thus, no coverage capability is lost by restricting candidate viewpoints to the MA. For clarity, boundary segments commonly observed by both \(p\) and the MA viewpoints (\(q\), or \(m\) and \(n\)) are not drawn.
    }
    \label{fig:proof_skeleton}
\end{figure}


\subsection{Global Minimal Cover--Connectivity on the Skeleton}\label{sec:global_optimality}

By Theorem~\ref{thm:extended_skeleton}, any coverage by interior points can be equivalently transferred to a suitable set of points on the medial axis. Hence, in the formulation~\eqref{eq:problem_formulation}, restricting $V$ to $\mathrm{MA}(P)$ (including any branch or joint nodes) captures all feasible coverage solutions.

\begin{theorem}[Global Minimal Cover--Connectivity]\label{thm:global_opt}
Let $S^*\subseteq \mathrm{MA}(P)$ be a minimal solution to~\eqref{eq:problem_formulation} that covers all $l_j\in L$ and satisfies the overlap-based connectivity requirement. Then $S^*$ is irreducible (i.e., removing any $v_i \in S^*$ breaks coverage or connectivity), and no smaller interior configuration can outperform $S^*$. Therefore, $S^*$ is \emph{globally optimal}.
\end{theorem}

\paragraph{Implication and Heuristic Search}
Exploiting the symmetry of the medial axis, no point \emph{outside} \(\mathrm{MA}(P)\) can provide superior coverage or connectivity. Consequently, a minimal cover--connectivity solution restricted to the skeleton cannot be improved by adding non-skeleton points. Hence, solving~\eqref{eq:problem_formulation} directly on \(\mathrm{MA}(P)\) yields a globally optimal arrangement in \(P\). Although the problem remains NP-hard, standard polynomial-time greedy algorithm (e.g.,~\cite{chvatal1979greedy}) often produce near-optimal results in practice. Once obtained, the minimal MA-based solution is irreducible, further affirming its global optimality for the entire polygon.


